Matrix Factorization-Based Clustering Of Image Features For Bandwidth-Constrained Information Retrieval

We consider the problem of accurately and efficiently querying a remote server to retrieve information about images captured by a mobile device. In addition to reduced transmission overhead and computational complexity, the retrieval protocol should be robust to variations in the image acquisition process, such as translation, rotation, scaling, and sensor-related differences. We propose to extract scale-invariant image features and then perform clustering to reduce the number of features needed for image matching. Principal Component Analysis (PCA) and Non-negative Matrix Factorization (NMF) are investigated as candidate clustering approaches. The image matching complexity at the database server is quadratic in the (small) number of clusters, not in the (very large) number of image features. We employ an image-dependent information content metric to approximate the model order, i.e., the number of clusters, needed for accurate matching, which is preferable to setting the model order using trial and error. We show how to combine the hypotheses provided by PCA and NMF factor loadings, thereby obtaining more accurate retrieval than using either approach alone. In experiments on a database of urban images, we obtain a top-1 retrieval accuracy of 89% and a top-3 accuracy of 92.5%.

==> Sections/Figures.tex <==
\begin{figure}[H]
\begin{centering}
\includegraphics[width=9cm]{Figures/topmatches_anglebw_subspaces}
\includegraphics[width=9cm]{Figures/topmatches_correlation}
\par\end{centering}

\caption{Plot of variation of Precision w.r.t the number of top matches considered.
when using different measures of error, (\ref{eq:score_PCA_basis})
and (\ref{eq:angle_NMF_subspaces}) for PCA and NMF.}


\end{figure}
\begin{figure}[H]
\begin{centering}
\includegraphics[width=9cm]{Figures/top1_rank}
\includegraphics[width=9cm]{Figures/top_20_rank}
\par\end{centering}

\caption{Variation of precision with model order, k, for the Top 1
and Top 20 matches considered. Horizontal lines represent the performance with the optimal rank selection.}


\end{figure}
\begin{figure}[H]
\begin{centering}
\includegraphics[width=9cm]{Figures/Quantization}
\par\end{centering}

\caption{Variation of Probability of finding the correct match among the top
20 images vs. Number of bits used to quantize the factor loading matrix.}


\end{figure}


\begin{figure}[H]
\includegraphics[width=9cm]{Figures/AlphaVsTop}

\caption{Variation of Precision with $\alpha$}


\end{figure}


\begin{figure}[H]
\includegraphics[width=9cm]{Figures/Matching}

\caption{Performance of NMF, PCA and Combined Schemes.}


\end{figure}


